Structural Operational Semantics for Control Flow Graph Machines

Compilers use control flow graph (CFG) representations of low-level programs because they are suited to program analysis and optimizations. However, formalizing the behavior and metatheory of CFG programs is non-trivial: CFG programs don't compose well, their semantics depends on auxiliary state, and, as a consequence, they do not enjoy a simple equational theory that can be used for reasoning about the correctness of program transformations. Lambda-calculus-based intermediate representations, in contrast, have well-understood operational semantics and metatheory, including rich equational theories, all of which makes them amenable to formal verification. This paper establishes a tight equivalence between (a variant of) Levy's call-by-push-value (CBPV) calculus and a control flow graph machine whose instructions are in static single assignment (SSA) form. The correspondence is made precise via a series of abstract machines that align the transitions of the structural operational semantics of the CBPV language with the computation steps of the SSA form. The target machine, which is derived from the CBPV language, accurately captures the execution model of control flow graphs, including direct jumps, mutually recursive code blocks, and multi-argument function calls, and the closure-free subset is similar to the SSA intermediate representations found in modern compilers such as LLVM and GCC. The definitions of all the language/abstract machine semantics and the theorems relating them are fully verified in Coq.

==> codegen.tex <==



% \subsection{Motivation}
%\dmitri{A potential summary, maybe of the entire approach: rather than
%adding syntactic restrictions to our source calculus to support
%``generating more efficient code'', we identify sufficient conditions
%for specialized instructions to be used within a more general
%compilation strategy.}

While the execution model described in the previous section is provides
reasonable cost model, and the virtual machine, by construction, are
similar to machines used in the compiler literature, there are clearly
CFG programs that are not in the image of the compilation
function. The most glaring omission is that we haven't yet accurately
captured mutually recursive blocks of code: since we've used CBPV's
negative products and projections to express mutual recursion, the
resulting CFG programs must push a projection argument and jump
through a $\kwl{SWI}  \,$ instruction. While we could modify
the CBPV language with a \code{letrec} construct directly, the
operational semantics of general \code{letrec} is itself nontrivial and the modified
compilation strategy of the previous section suggests an alternative.

Thus far, our goal was to have the CFG machine and the CBPV semantics implement the same transition system, modulo the syntax of
states. In the CFG machine, rather than pushing a statically known projection and then executing a $\kwl{SWI}  \,$ instruction, we could easily write a program that jumps directly to the target; however, there is no single SOS reduction rule that will
eliminate a thunk and tuple at once. 
% While including \code{letrec} in applied functional languages is standard, there are increasingly more complicated constructs that arise with mutual recursion and function pointers, and
% it would be unreasonable to extend the source calculus for each
% instruction we might want to add to our execution model.
% It's even
% less desirable when, as in the case of \code{letrec}, we can already
% express our intended semantics with a series of reductions. 
In this section, we describe a general technique for using machine instructions that do not correspond to a single reduction in the SOS rules, while retaining the tight correspondence between execution models.

\subsection {Annotations for code generation.}
\label{sec:annotations}
The overall approach is to add ad-hoc\steve{are they ad-hoc?} annotations to the
source language to control the associated execution model without
changing the source semantics. Many real compiler intermediate
representations include an interface for communicating additional
non-semantic information to the code generation phase; our approach
can be seen as an attempt to formalize this process. At the CBPV level,
the annotations give rise to an SOS in which annotated terms take larger steps;
at the CFG level, they allow more efficient compilation, removing some of the potentially undesirable features of straightforward translation from CBPV. We have used this
approach to enable our cost model for CBPV terms to include mutually
recursive blocks of instructions both with and without intervening
dispatch using $\kwl{SWI}  \,$ instructions.

%% \input{temp/fig-mkargs}

\paragraph {Extending the compiler.}
The only required change to our CBPV language is to allow terms to be
tagged with some additional annotations. To support direct jumps under
tuples, this is just an extra flag on projections $ \overline{ \kw{prj} }_{ \ottmv{n} }\;  \ottnt{M} $
indicating that reduction happens, for the purposes of the cost
model, at compile time. At the CFG level, when compiling a $ \kw{force} $, we
may take advantage of these annotations: if the target of the jump is a label, we examine
the context for any immediately enclosing compile-time projections and
execute them immediately, removing them from the generated $ \kw{args} $ and
extending the target label to skip over the associated tuples/$\kwl{SWI}  \,$ instructions. Aside from this modification,
the compiler is unchanged from Section \ref{sec:cfg1} and has been
omitted for space. % Please refer to the accompanying Coq development for
% details. \william{Do we want to say that?}

\paragraph {Well-annotated terms and correctness.}
The optimized compilation strategy described above does not provide useful output for every possible annotated term.
It ignores compile-time projections that
do not occur immediately above a $ \kw{force} $, and if the source term gets stuck then it may produce
jumps to undefined paths (which never occurred in the original compiler). It would be very
difficult to reason about the results of this compilation strategy for
arbitrary annotated terms, without accounting for the specifics of the
compilation strategy. Instead, we define a subset of CBPV terms which we call ``well-annotated'', for which all annotations will be compiled correctly.
% \todo{Too informal?} \steve{No!}
\begin{definition}
  A term $\ottnt{M}$ is well-annotated iff
  \begin{enumerate}
  \item Sequences of compile-time projections only occur directly
  above a $ \kw{force} $, and
  \item The target of such a $ \kw{force} $ is either a $\texttt{\textcolor{red}{<<no parses (char 1): r***ec >>}}$ or a variable
  bound by a $\texttt{\textcolor{red}{<<no parses (char 1): r***ec >>}}$, and the $\texttt{\textcolor{red}{<<no parses (char 1): r***ec >>}}$ immediately encloses a set of nested tuples for
  which the projections are valid.
  \end{enumerate}
\end{definition}
Note that terms not containing annotated projections are trivially
well-annotated. We augment the SOS with the following rule:
\[
\begin{array}[t]{lr@{\ \  \longrightarrow  \ \ }l}
\rn{\overline{prj}} &  \overline{ \kw{prj} }_{ \ottmv{i} }\;  \ottnt{M}  & \ottnt{M_{\ottmv{i}}} 
\qquad \hfill \mbox{if $\ottnt{M}  \longrightarrow  \langle  \ottnt{M_{{\mathrm{1}}}}  \ottsym{,} \, .. \, \ottsym{,}  \ottnt{M_{\ottmv{n}}}  \rangle$} \\
\end{array}
\]
It is not necessary to specify whether the usual search and reduction
rules for projections apply to the compile-time annotated variant,
since those cases never arise in well-annotated terms. The statement
of correctness is identical to Theorem \ref{compile-correct} restricted
to well-annotated terms, where the operational semantics are
augmented with the rule above, and the optimized compilation strategy
is used.

%% \paragraph {Other optimizations.}
%% We conjecture that this technique can support various ad-hoc
%% extensions to our CBPV-CFG correspondence. We have formulated (but not
%% yet verified) methods of adding the following features using code-generation
%% annotations: 
%% \begin{itemize}
%% \item Specializing direct tail calls into parallel move
%% instructions. Many real compiler intermediate representations
%% differentiate between tail calls and jumps within a machine procedure,
%% and this optimization is a step towards a more literal implementation
%% of \kw{phi} nodes.
%% \item Specializing the case where a
%% variable bound by a $\texttt{\textcolor{red}{<<no parses (char 1): r***ec >>}}$ only appears under a $ \kw{force} $ within its
%% scope. This corresponds to omitting the function preamble.
%% \item Expressing function pointers, including those to
%% mutually-recursively defined functions, as bare labels when it's
%% syntactically apparent that the definitions do not close over any free
%% variables.
%% \end{itemize}
%% These are typically optimizations done using analyses on low-level
%% intermediate representations.

%% Local Variables:
%% fill-column: 70
%% eval: (auto-fill-mode)
%% eval: (flyspell-mode)
%% eval: (setq-local auto-hscroll-mode nil)
%% eval: (setq-local sentence-end-double-space nil)
%% End:


==> comparison.tex <==
The final form of the CFG virtual machine that we consider in this
work strays from typical SSA intermediate representations in a
number of ways. Most importantly, we claim that it accurately models
key aspects of the execution of the intraprocedural fragment most
commonly targeted by optimizations. We argue informally, but also
consider what it might mean to prove this property.

\subsection{Extensions}
%% Mention opret, trivial
The most obvious extension to SSA form in our machine is that labels
can appear as arguments to non-arithmetic instructions, and they allocate
closures when evaluated. It's worth noting how small of a change this
is: operational semantics given for full SSA languages~\cite{vellvm,compcertssa} already allocate closures to model the stack
frame.

Next, the use of the argument stack is more flexible than usual
formulations of SSA. We conjecture that the restrictions present in
SSA and functional IRs using multi-argument functions can be
reintroduced by requiring that lambdas only appear directly under a
$\texttt{\textcolor{red}{<<no parses (char 1): r***ec >>}}$ and are never sequenced. However, this would rule out use of
the argument stack for defining variable-argument functions. We
believe these are useful for, among other things, efficiently
representing curried functions when compiling ML-family languages to
CBPV. The accompanying Coq development contains versions of the
\code{eval} combinators~\cite{marlow04} implemented in our CBPV
fragment.

The $\kwl{SWI}  \,$ instruction is a form of jump-table instruction that is
not commonly considered in CFG machines. Intuitively, it can be
thought of as a control-flow analog of SSA's phi functions: each
control flow predecessor of a block containing a $\kwl{SWI}  \,$ must
have an associated projection on which to dispatch as well as
arguments bound by phi nodes. Within a single function, it
allows sharing a prefix of a block between CFG
predecessors while requiring the associations to be statically known.
It can always be rewritten by making a copy of the shared section of
the CFG for each control flow predecessor. For our full language,
where the control flow predecessor of a block is not always known,
$\kwl{SWI}  \,$ supports a form of dynamic dispatch, where ``messages'' are
kept distinct from runtime values.

\subsection{Future Work}
As we alluded to in Section \ref{sec:annotations}, CFG representations
typically distinguish between ``machine procedures'' and
intraprocedural control flow. While semantically both can be
represented by functions, the distinction is important for code
generation and optimization. Machine procedures require generating a
function preamble implementing a standard parameter passing protocol,
while SSA basic blocks do not. The key difference is that SSA block
labels are assumed not to escape, and code generation can assume that
every call site is known and can be specialized. Previous work
on the SSA-functional programming correspondence only makes claims
about a syntactically restricted first-order subset of functional
programs~\cite{kelseyssa,BeringerMS03,SchneiderSH15}. We extend the
correspondence to higher-order programs. Our CFG instruction set
similarly contains both $ \kwl{MOV} $ instructions and tail calls, and both
can represent SSA phi functions by merging values at control flow join
points, but our compiler only emits the former in simple cases. We
have sketched an approach for using our code-generation annotations to
distinguish additional intraprocedural control flow without
modifying the source language.

While SSA intermediate representations do not typically include
closures as primitive values \dmitri{[MLTON may be an exception]}, they do
include function pointers. Our CFG machine currently only supports
passing code values as closures. We believe that explicitly omitting
allocating empty environments for closures that correspond to uses of
function pointers in standard SSA is possible using our technique.
\todo {Particular form of the conditional statement omitting extra jumps?}
\dmitri {We should just rewrite the SSA example to use separate branch/jump} 

\subsection{Completeness}
A natural question to consider is whether our CBPV-CFG correspondence
can be used to reason about any SSA program, or whether there are
useful programs not in the image of our compilation function.
This is a difficult property to state precisely, since it is dependent
on the particular form of instructions chosen, and there is no
canonical choice for SSA. We do claim, however, that there is a subset
of CBPV terms that intuitively correspond to the intraprocedural
fragment of SSA, for which our SOS and CFG machine accurately capture
the intended semantics and execution model. 

Consider the subset of well-annotated terms that contain only
compile-time projections, where $\texttt{\textcolor{red}{<<no parses (char 1): r***ec >>}}$ and variables bound by
$\texttt{\textcolor{red}{<<no parses (char 1): r***ec >>}}$ only occur directly under $ \kw{force} $. We also require that
lambdas only appear directly under tuples, the root of the
term, or other lambdas, and that only arithmetic operations appear in
the left position of a sequence. The example in Fig.~\ref{fig:ssacfg}
is such a program along with its compiled CFG. It is clear by
inspection that our compilation function will not emit calls with
projection arguments, or any instructions that allocate closures.
Furthermore, we can express arbitrary CFGs, modulo our particular
choice of conditional instruction.
\dmitri{Should I try to write a grammar?}\steve{Isn't this exactly
a ``syntactic restriction''?  Maybe not if the subset is closed under
reduction in the CBPV language.}

A related question is whether it is possible to express all reasonable CFG
programs as CBPV terms. In Section~\ref{sec:codegen} we showed that
this is not the case, and provided several examples of CFG programs
that are not in the image of the compilation function. For instance, 
the compiler only produces a subset of terms that use $ \kwl{MOV} $
instructions at control flow join points, since they are only emitted
for $ \kw{prd} $ to the immediately enclosing sequence. One goal
might be to characterize well-formed control flow graphs directly,
rather than as the image of our compilation function. It would be
interesting to formulate the higher-order variant of the SSA dominator
condition, but we leave such considerations to future work.

% \paragraph{Administrative normal forms}
% A common intermediate representation used by function compilers
% is \textit{administrative normal form}, or ANF. ANF programs are
% lambda calculus terms with explicit \code{let} bindings, normalized
% with respect to a set of rewrite rules derived from the call-by-value
% CPS transformation. A-normalization limits the form of evaluation
% contexts, so that terms can be evaluated by a machine that only
% maintains a stack of return continuations for non-tail calls
% [Felleisen]. Fig. \ref{fig:anf} shows a the example program from
% Section~\ref{problem} as an ANF procedure.

% When applied, an ANF machine will first bind mutually recursive
% closures for \code{f} and \code{g} which contain additionally the
% arguments\code{m} and \code{n}. To invoke the tail call under the let,
% it will then look up \code{f} in the environment and invoke the
% closure, restoring the previously saved environment. Since ANF is
% higher order, the bound functions \code{f} and \code{g} may escape,
% and therefore represented in such a way that they could be returned as
% values from the procedure. 


% "Can't you follow the same approach with ANF?" \\
% * CBPV source already has the necessary sequencing information \\
% * ANF not closed under beta \\ 
% * CPS is closed under beta, but CBV/CBN split doesn't exist for CBPV \\
% * ANF requires extensions to handle multi-arg calls and mutrec \\
% * can't you deal with extensions using the same annotation approach? (?)\\
% %% 
% %
% \begin{figure}
% \begin{lstlisting}[columns=flexible,language=ANF]
% lambda n m.
%   let rec f = lambda m a.
%     if0 m then a
%     else
%       let m' = m - 1 in
%       g(a, 0, m')
%   and g = lambda m a m$_k$.
%     if0 m then f(m$_k$, a)
%     else
%       let m' = m - 1 in
%       let a' = a + n in
%       g(m', a', m$_k$)
%   in f(m, 1)
% \end{lstlisting}
% \caption{ANF program that computes $n^m$ via repeated addition.}
% \label{fig:anf}
% \end{figure}
%
%% Local Variables:
%% fill-column: 70
%% eval: (auto-fill-mode)
%% eval: (flyspell-mode)
%% eval: (setq-local auto-hscroll-mode nil)
%% eval: (setq-local sentence-end-double-space nil)
%% End:


==> fig-cekfuns.tex <==
%% CEK
\begin{figure}[t]
\[
\begin{array}[t]{r@{\ }l@{\ \ }c@{\ }lll}
  \mathrm{State} \ \ni\ & \sigma & =\  & \mathrm{Term} \times \mathrm{Env}
\times \mathrm{Kont} \\
  %% \mathrm{Term} \ \ni\ & \ottnt{c} & \bnf\ & \ottnt{M} \\
  %% \mathrm{Env} \ \ni\ & \ottnt{e} & =\ & \mathrm{Var}
  %%   \longrightarrow_{\mathrm{fin}} \mathrm{Val} \\
  \mathrm{Env} \ \ni\ & \ottnt{e} & \bnf\ & \cdot
    \sep \ottsym{[}  \ottmv{x}  \mathbin{\mapsto}  \ottnt{v}  \ottsym{]}  \ottnt{e}
    \sep \ottsym{[}  \ottmv{x_{{\mathrm{1}}}}  \mathbin{\mapsto}  \ottnt{M_{{\mathrm{1}}}}  \ottsym{,} \, .. \, \ottsym{,}  \ottmv{x_{\ottmv{n}}}  \mathbin{\mapsto}  \ottnt{M_{\ottmv{n}}}  \ottsym{]}  \ottnt{e}\\
  \mathrm{Kont} \ \ni\ & k & \bnf\ & \cdot \sep  \ottnt{v}  \mathbin{\cdot} \, \underline{\ \ } :: \ottnt{k} 
    \sep  \ottsym{[} \, \underline{\ \ } \, \kw{to} \, \ottmv{x} \, \kw{in} \, \ottnt{M}  \ottsym{,}  \ottnt{e}  \ottsym{]} :: \ottnt{k}  \\
  %% TODO: errors?
  \mathrm{DVal} \ \ni\ & v & \bnf\ & \ottmv{x} \sep \ottsym{[}  \ottnt{M}  \ottsym{,}  \ottnt{e}  \ottsym{]}
\end{array}
\]
\vspace{5mm}
  \[
  \begin{array}{rcl}
    \gamma & : & \mathrm{Val} \rightarrow \mathrm{Env} \rightarrow \mathrm{DVal} \\
     \gamma\;  \ottmv{x} \;  \ottnt{e}  & = & \mathrm{lookup}(\ottnt{e}, \ottmv{x}) \\
    %%  \gamma\;   n  \;  \ottnt{e}  & = & \ottmv{n} \\
     \gamma\;  \ottsym{(}  \kw{thunk} \, \ottnt{M}  \ottsym{)} \;  \ottnt{e}  & = & \ottsym{[}  \ottnt{M}  \ottsym{,}  \ottnt{e}  \ottsym{]} \\
  \end{array}
  \]
  \caption{CEK syntax and value-semantics function $ \gamma $.}
  \label{fig:cekfuns}
\end{figure}


==> fig-mkargs.tex <==
\begin{figure}[t]
\noindent
\begin{lstlisting}[basicstyle={\sffamily},mathescape=true]
    $\kw{argsH}$ $a$ = 
    match $a$ with
    | $\cdot$ $\TO$ ($\cdot$, $\kw{none}$)
    | $  \kwl{ARG}\; \ottnt{p}   ::  a' $ $\TO$ 
      $\kw{map}_{\times}\;(\kw{fun}\;l\;\TO  \kwl{ARG}\; \ottsym{(}  \overline{\gamma} \, \ottsym{(}   \ottsym{0}  \CONS  \ottnt{p}   \ottsym{)}  \ottsym{)} ::l)\;\kw{id}\; (\kw{argsH}\;a'$)
    | $ \kwl{PRJ} \, \ottmv{i}  ::  a' $ $\TO$ 
      $\kw{map}_{\times}\;(\kw{fun}\;l\;\TO \kwl{PRJ} \, \ottmv{i}::l)\;\kw{id}\; (\kw{argsH}\;a'$)
    | $ \kwl{SEQ} \, \ottnt{p}  ::  a' $ $\TO$ ($\cdot$, $\kw{some}$ $a'$)
    end

    $\kw{args} \, \ottnt{p}$ = $\kw{argsH}\ (\kw{aframes} \, \ottnt{p})$
\end{lstlisting}
  \caption{$ \kw{args} $ compiler function.}
  \label{fig:mkargs}
\end{figure}


==> notes.tex <==
\subsection{Introduction}
\steve{Here are some of my thoughts related to the introduction. I'm
  writing them down mostly to help organize them and explain this to
  myself.  We probably don't need to include too much of this, but
  maybe it can help.}

\paragraph{SOS}
Structural operational semantics: transition system whose states are
just the terms of the language (at least for the pure parts of a
computation). Evaluation described in terms of meta-level operations
(primarily substitution). Evaluation order and control-flow determined
by meta-level constraints on the terms (i.e. side conditions about
which terms count as values) and congruence rules that ``search'' for
the next redex. Substitution plus congruence rules give rise to an
equational theory that directly captures the abstract idea of
``replacing equals by equals''. Pros: compositional, structured, easy
to work with because everything is uniformly represented as a term,
equational theory makes specifying/understanding/implementing many
semantics-preserving program transformations easy. Cons: meta-level
substitution is far removed from hardware models, costs (e.g.
space/time) not entirely apparent because of the abstraction.

\paragraph{Abstract machines}
Abstract machines: transition system whose state consists of a term
plus additional data structures that implement substitution
(environments, closures) and the search rules (a stack). These extra
state components move substitution and the congruence rules that
embody search from the meta-level to the object level. Abstract
machines use simpler meta-level operations of environment lookup and
stack push/pop. But still require complex meta-level inspection of the
term to determine the control behavior (i.e. you have to pattern match
against the structure of the term to take it apart and determine which
rule of the operational semantics to apply). Pros: suitable for
efficient interpreters since the ``meta-level'' operations are more
explicit; because the ``control'' of the machine is still given by a
high-level term, the connection to the (initial) source program is
clear. Cost model is more apparent; for example differences between
stack usage can be observed here (call vs tailcall). Cons: Less
compositional (i.e. there's no notion of substituting one abstract
machine for a part of another abstraction machine), though one could
substitute through the control. Intermediate states are less obviously
connected to the source.  This is less ``pure'' because it introduces
additional state components. 

\paragraph{Virtual machines}
Virtual machines: Like abstract machines, a virtual machine's state
includes an explicit representation of the environment (often thought
of as a register file). Unlike abstract machines, they have an
instruction set and hence require compilation. Major distinction:
factoring the program's representation into its purely static parts,
namely the code of the program, and its dynamic parts: a ``program
counter,'' the environment, and a stack. In contrast to abstract
machines, the compilation step means that the meta-level dispatch on
which evaluation step to apply is determined locally by information
entirely contained in the instruction. Pros: Apart from assuming an
infinite number of ``registers,'' and the particular details of the
instruction set; virtual machines are close closer to the
``hardware.'' Especially w.r.t. cost semantics. Meta-level function of
\kw{next\_path} (i.e. incrementing the PC) is implementable in
constant time. 
Cons: least compositional, since compilation does not,
in general, commute with substitution (especially since the compiler
tries to take advantage of known calls, etc.).  

Virtual machine code is often structured as control-flow-graph.
Classic compiler analysis and transformation passes work with CFG
representation.   SSA?

\paragraph{Closures conversion} Most SSA-level languages for C
compilers stick to ``first order.'' i.e. although they have code
pointers, closures would need to constructed by explicitly allocating
heap structures / copying the environment.  Our version of SSA
includes closures explicitly in the machine semantics---this makes our
SSA language one step removed from languages like LLVM.

\paragraph{Effects} The discussion above assumes that the language has
no ``world effects'' (e.g. heap, I/O). Adding them can complicate the
story about the equational theory for SOS. Adding such effects to CBPV
is comparatively straightforward---its monadic structure is already
conducive to such extensions. The correspondence between steps of the
CBPV SOS and the SSA machine preserves all of the behaviors of the
source program (so any behavioral equivalence determined by observing
effects at the CBPV level should directly port to a corresponding
equivalence at the SSA level). \steve{Need to think more about how to
  present this part of the story.}

\paragraph{What this paper is about.} This paper establishes a machine
equivalence between CBPV and a ``low-level'' SSA language based on
control-flow-graphs. Because this is an \textit{equivalence} and not a
one-way refinement relation, you can think of it in two ways:

\begin{itemize}
\item On the one hand, this result can be thought of as a way to
  translate CBPV into a low-level SSA/LLVM-like representation.  This
  means that compilers for functional languages could use this as a
  compilation path more or less like: $\lambda$ $\to$ CBPV $\to$ CFG.
  If one wanted to translate ML or Haskell to LLVM, perhaps to take
  advantage of its many backends, this would be a reasonable thing to
  do. 

\item On the other hand, the correspondence also shows that rather
  than manipulated control-flow-graphs directly, one could
  equivalently design a compiler to work on CBPV terms.  Using CBPV
  terms rather than control-flow-graphs as the intermediate
  representation could be useful for several reasons. As in
  discussion above, the SOS of CBPV enjoys substitution and
  well-studied equational theory that may make expressing some
  optimizations easier.  It also means that class compiler techniques
  (like dataflow analysis) can potentially structured as type systems,
  which have also been well-studied in the literature.

  \steve{To make this second approach work for existing LLVM-like
    compilers, we would need a completeness result saying how to unload
    arbitrary CFGs back into CBPV terms.}
\end{itemize}

\steve{One of the things I think that we've been struggling with when
  trying to write this paper is which of the two views above is the
  ``one'' we want to present.  Perhaps we should just put both of them
forward?  The second is a bit more speculative in some ways.  Parts of
the motivation the Dmitri has been thinking about are related to the
first point: i.e. efficient compilation of curried/multi-argument
functions, etc.}


==> preamble.tex <==
\usepackage{xypic}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{tikz} %commutativity diagrams
\usetikzlibrary{arrows}
\usepackage{etoolbox} % replaces ifthen package
\AtBeginEnvironment{alltt}{\setlength{\topsep}{2pt}}
\usepackage[capitalize,noabbrev]{cleveref}
\usepackage{mathtools} % xarrow extensions
\usepackage{supertabular}
\usepackage{listings}
\usepackage{multirow}
\lstset{
  language=[Objective]Caml,
  basicstyle=\ttfamily
}

\RequirePackage{proof}

\newcommand{\cd}[1]{\lstinline[backgroundcolor=\color{white}]$#1$}


% Fixing the fonts introduced by the eptcs class
\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n}
% From the `lmodern` package
\DeclareSymbolFont{lsymbol}{OML}{lmsy}{m}{n}

\makeatletter
\begingroup
\count@=0
\loop
\edef\DOIT{%
 \noexpand\DeclareMathSymbol
   {\expandafter\noexpand\ifcase\count@
         \Gamma   \or \Delta \or \Theta   \or \Lambda
     \or \Xi      \or \Pi    \or \Sigma   \or \Upsilon
     \or \Phi     \or \Psi   \or \Omega
     %
     \or \alpha   \or \beta  \or \gamma   \or \delta
     \or \epsilon \or \zeta  \or \eta     \or \theta
     \or \iota    \or \kappa \or \lambda  \or \mu
     \or \nu      \or \xi    \or \pi      % We skip \omicron
     \or \rho     \or \sigma \or \tau     \or \upsilon
     \or \phi     \or \chi   \or \psi     \or \omega
   \fi}%
   {\noexpand\mathalpha}%
   {lsymbol}%
   {\the\count@}%
}
\DOIT
\advance\count@ by 1
\ifnum\count@<34
\repeat
\endgroup
\makeatother
% fin

% Formatting
\usepackage{xspace}
\usepackage{multicol}
\usepackage{color}
\usepackage{alltt} % verbatim
\usepackage{enumerate}

% Proof Trees
\usepackage{mathpartir}
%% \usepackage{bussproofs}
%% \EnableBpAbbreviations
%% \newcommand{\END}[1]{\AXC{~} \UIC{#1}}
%% \usepackage[inference]{semantic}

% Symbols
\usepackage{cmll} % Linear logic symbols
\usepackage{stmaryrd} % llbracket, rrbracket
\usepackage{mathtools} % xRightArrow
%% \usepackage{mathabx}
%% \usepackage{latexsym}
%% \usepackage{textcomp}
%% \usepackage{bbold} % mathbb extended
%% \usepackage{harpoon} % harpoon
%% \usepackage{MnSymbol} % harpoon, brackets

% Bibliography
%\usepackage[numbers]{natbib}
%\bibpunct();A{},
%\let\cite=\citep
%\newcommand{\citep}[1]{\fixme{\cite{#1}}}
%\newcommand{\citet}[1]{\fixme{\cite{#1}}}
%\newcommand{\citeyearpar}[1]{\fixme{\cite{#1}}}

% ``English''
\newcommand{\nary}{\hbox{n-ary}\xspace}
\newcommand{\eg}{\textit{e.g.}\xspace}
\newcommand{\ie}{\textit{i.e.}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\etal}{~\textit{et al.}\xspace}

% References
\newcommand{\Figure}[1]{Figure~\ref{fig:#1}}
\newcommand{\Section}[1]{Section~\ref{sec:#1}}
\newcommand{\Lemma}[1]{Lemma~\ref{lem:#1}}
\newcommand{\Theorem}[1]{Theorem~\ref{thm:#1}}
\newcommand{\Proposition}[1]{Proposition~\ref{prop:#1}}
\newcommand{\Corollary}[1]{Corollary~\ref{cor:#1}}
\newcommand{\Conjecture}[1]{Conjecture~\ref{conj:#1}}
\newcommand{\Definition}[1]{Definition~\ref{def:#1}}

% Theorems and Lemmas
%% \newtheorem{theorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
%% \newtheorem{lemma}[theorem]{Lemma}
%% \newtheorem{proposition}[theorem]{Proposition}
%% \newtheorem{corollary}[theorem]{Corollary}
%% \newtheorem{conjecture}[theorem]{Conjecture}
%% \newtheorem{definition}[theorem]{Definition}
\newenvironment{unfinishedproof}{\paragraph{Proof:}}{\hfill$\boxtimes$}

% Table formatting
\newcommand{\ltwo}[1]{\multicolumn{2}{l}{#1}}
\newcommand{\ctwo}[1]{\multicolumn{2}{c}{#1}}

% General formatting
\newenvironment{aside}{\begin{quote}NOTE: \itshape}{\end{quote}}
\newcommand{\bslash}{\textbackslash}

% Fonts
\newcommand{\longcatfont}[1]{\textsc{#1}\xspace}
\newcommand{\catfont}[1]{\mathcal{#1}}
\newcommand{\functorfont}[1]{\mathrm{#1}\xspace}
\newcommand{\arrowfont}[1]{\mathit{#1}\xspace}
\newcommand{\objectfont}[1]{\mathit{#1}\xspace}
\newcommand{\tc}[1]{\textup{\textsf{#1}}}   % type constructors
\newcommand{\kw}[1]{\textup{\textbf{\textsf{#1}}}}   % keywords
\newcommand{\kwl}[1]{{\small\textup{\texttt{#1}}}}   % lightweight keywords
\usepackage[T1]{fontenc}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\confont}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\meta}[1]{\textrm{\textit{#1}}}
\newcommand{\rn}[1]{\ensuremath{\mathit{#1}}}

% Category Theory
\newcommand{\cat}[1]{\catfont{#1}}
\newcommand{\functor}[1]{\functorfont{#1}}
\newcommand{\obj}[1]{\objectfont{#1}}

\newcommand{\op}[1]{{#1}^{op}}
\newcommand{\inv}[1]{#1^{-1}}
\newcommand{\id}[1]{\arrowfont{id}_{#1}}


% Sets
\newcommand{\union}{\mathbin{\cup}}
\newcommand{\inter}{\mathbin{\cap}}
\newcommand{\powerset}[1]{\mathcal{P}(#1)}
\newcommand{\eqdef}{\ensuremath{\triangleq}}
\newcommand{\namedfun}[2]{\ensuremath{\textrm{#1}(#2)}}

% Multisets
\newcommand{\lmultiset}{\ensuremath{\{\!\!\{}}
\newcommand{\rmultiset}{\ensuremath{\}\!\!\}}}
\newcommand{\mset}[1]{\ensuremath{\lmultiset #1 \rmultiset}}
\newcommand{\munion}{\Cup}
\newcommand{\minter}{\Cap}
\newcommand{\msub}{\Subset}
\newcommand{\mcard}[1]{\ensuremath{|#1|}}
\newcommand{\mfact}[1]{\ensuremath{#1!}}
\newcommand{\mdiff}{\ensuremath{-}}




% Standard mathematical definitions
% Field
\newcommand{\F}{\ensuremath{\mathbb{F}}\xspace}
% Integers
\newcommand{\Z}{\ensuremath{\mathbb{Z}}\xspace}
% Naturals
\newcommand{\N}{\ensuremath{\mathbb{N}}\xspace}
% Rationals
\newcommand{\Q}{\ensuremath{\mathbb{Q}}\xspace}
% Reals
\newcommand{\R}{\ensuremath{\mathbb{R}}\xspace}
% Complex
%% \newcommand{\C}{\ensuremath{\mathbb{C}}\xspace}


% Math
\newcommand{\dom}[1]{\namedfun{dom}{#1}}
\newcommand{\meanl}{\ensuremath{[ \! [}}
\newcommand{\meanr}{\ensuremath{] \! ]}}
\newcommand{\means}[1]{\ensuremath{\meanl #1 \meanr}}
\newcommand{\meansE}[1]{\ensuremath{\mathcal{E}\meanl #1 \meanr}}
\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\interp}[1]{[ #1 ]}
%\newcommand{\interpalt}[1]{\langlebar #1 \ranglebar}
%\newcommand{\interpalt}[1]{\llangle #1 \rrangle}
%\newcommand{\interpalt}[1]{\llparenthesis #1 \rrparenthesis}
%\newcommand{\interpalt}[1]{\lgroups #1 \rgroups}
\newcommand{\interpalt}[1]{\llbracket #1 \rrbracket}

\newcommand{\E}{\mathcal{E}}
\newcommand{\setof}[1]{\left\{#1\right\}}
\newcommand{\comprehend}[2]{\setof{{#1}\;\middle|\;{#2}}}


% Proof Theory and Programming Languages
\newcommand{\shows}{\ensuremath{\vdash}}

% General PL
\newcommand{\typed}{\ensuremath{\mathord{:}}}
\newcommand{\hastype}{\ensuremath{\mathrel{:}}}

\newcommand{\TO}{\ensuremath{\Rightarrow}}
\newcommand{\bnf}{::=}
\newcommand{\sep}{\ \ \ensuremath{\mid} \ \ }
\newcommand{\fv}[1]{\namedfun{fv}{#1}}
\newcommand{\bv}[1]{\namedfun{bv}{#1}}
\newcommand{\LET}{\kwfont{let}}
\newcommand{\IN}{\kwfont{in}}
\newcommand{\letin}[3]{\LET \; #1 = #2 \; \IN \; #3}
\newcommand{\INJ}{\kwfont{in}}
\newcommand{\inj}[2]{\ensuremath{\INJ_{#1}^{#2}}}
\newcommand{\FIX}{\kwfont{FIX}}
\newcommand{\fix}[2]{\ensuremath{\FIX \; #1.\; #2}}
\newcommand{\CASE}{\kwfont{case}}
\newcommand{\OF}{\kwfont{of}}
\newcommand{\patto}{\ensuremath{\mapsto}}
\newcommand{\caseof}[5]{\CASE \; #1 \; \OF \; \inj{1}{} \; #2 \patto #3
                                 \mid \inj{2}{} \; #4 \patto #5}
\newcommand{\subst}[3]{#1\{#2 / #3\}}

% Logic
\newcommand{\IMPLIES}{\ensuremath{\Longrightarrow}}
\newcommand{\OR}{\ensuremath{\vee}}
\newcommand{\AND}{\ensuremath{\wedge}}
\newcommand{\NOT}{\ensuremath{\neg}}
\newcommand{\IFF}{\ensuremath{\Longleftrightarrow}}
\newcommand{\IF}{\kwfont{if}\xspace}
\newcommand{\THEN}{\kwfont{then}\xspace}
\newcommand{\ELSE}{\kwfont{else}\xspace}
\newcommand{\ift}[3]{\ensuremath{\IF\ {#1} \ \THEN\ {#2} \ \ELSE\ {#3}}\xspace}

% Linear Logic Connectives
\newcommand{\mprod}{\mathbin{\text{\footnotesize \ensuremath{\otimes}}}}
\newcommand{\aprod}{\mathbin{\text{\footnotesize \ensuremath{\&}}}}
\newcommand{\msum}{\mathbin{\text{\footnotesize \ensuremath{\parr}}}}
%\newcommand{\msum}{\shortparallel}
\newcommand{\asum}{\mathbin{\text{\footnotesize \ensuremath{\oplus}}}}
\newcommand{\lolto}{\ensuremath{\multimap}}
\newcommand{\bang}{\ensuremath{\oc}}
\newcommand{\whynot}{\ensuremath{\wn}}
\newcommand{\one}{\ensuremath{1}}
\newcommand{\zero}{\ensuremath{0}}

\newcommand{\lollialt}{\ensuremath{\mathrel{\multimap\mkern-14mu\bullet}}}

\newcommand{\dualize}[1]{\ensuremath{{#1^{\bot}}}}
\renewcommand{\vec}[1]{\overrightarrow{#1}}

\newcommand{\typename}[1]{\textit{#1}}
\newcommand{\funname}[1]{\texttt{#1}}
\newcommand{\kwoperator}[1]{\operatorname{\kwfont{#1}}}

\newcommand{\tbot}{$\bot$}


% Semantics
\newcommand{\norm}[1]{\kwfont{normalizes}(#1)}
\newcommand{\Ok}[1][]{\mathrm{Ok}_{#1}}
\newcommand{\Stable}[1][]{\mathrm{Good}_{#1}}
\newcommand{\Store}{\mathrm{Store}}
\newcommand{\Config}{\mathrm{Config}}
\newcommand{\Expr}{\mathrm{Expr}}
\newcommand{\store}{\sigma}
\newcommand{\Loc}{\mathrm{Loc}}
\newcommand{\dsum}[2]{\Sigma{#1}.\;{#2}}
\newcommand{\Multiset}[1]{\mathcal{M}(#1)}
\newcommand{\Val}{\mathrm{Val}}
\newcommand{\Heap}{\mathrm{LinearHeap}}
\newcommand{\Event}{\mathrm{Event}}
\newcommand{\Callbacks}{\mathcal{C}}
\newcommand{\config}[2]{\left\langle{#1}; {#2}\right\rangle}
\newcommand{\eval}[4]{\config{#1}{#2} \Downarrow \config{#3}{#4}}
\newcommand{\chan}{\mathrm{chan}}
\newcommand{\Chan}{\mathrm{Chan}}

\newcommand{\step}[3][]{{#2} \Longrightarrow^{#1} {#3}}
\newcommand{\stepaux}[4]{ {#1} \vdash_{#2} {#3} \leadsto {#4}}

\newcommand{\Perm}{\mathrm{Perm}}
\newcommand{\Res}{\mathrm{Res}}
\newcommand{\Safe}{\mathrm{Safe}}
% \newcommand{\N}{\mathbb{N}}
\newcommand{\bnfalt}{\;\;|\;\;}
\newcommand{\FL}[1]{\mathrm{FL}(#1)}
\newcommand{\FV}[1]{\mathrm{FV}(#1)}
\newcommand{\supported}[1]{{#1}\;\mathrm{supp}}
\newcommand{\supp}[2]{{#1} \sqsubseteq {#2}}

\newcommand{\fun}[2]{\lambda {#1}.\;{#2}}
\newcommand{\allttfun}[2]{\(\lambda\){#1}.{#2}}
\newcommand{\ttdiamond}{\(\diamond\)}
\newcommand{\tttensor}{\(\otimes\)}
\newcommand{\ttlolli}{\(\lolto\)}
\newcommand{\unit}{\left\langle\right\rangle}
\newcommand{\pair}[2]{\left\langle{#1}, {#2}\right\rangle}
\newcommand{\prj}[2]{\pi_{#1}\,{#2}}
% \newcommand{\inj}[2]{\mathsf{in{#1}}({#2})}
\newcommand{\inl}[1]{\mathsf{inl}({#1})}
\newcommand{\inr}[1]{\mathsf{inr}({#1})}
\newcommand{\case}[5]{\mathsf{case}({#1}, \inl{#2} \to {#3}, \inr{#4} \to {#5})}
\newcommand{\newref}[1]{\mathsf{new}({#1})}
\newcommand{\letv}[3]{\mathsf{let}\; {#1} = {#2} \mathsf{\;in\;} {#3}}
\newcommand{\attach}[2]{\mathsf{attach}({#1}, {#2})}
\newcommand{\invoke}[2]{\mathsf{invoke}({#1}, {#2})}

\newcommand{\Infer}[3]{\inferrule*[right={#1}]{#2}{#3}}

\newcommand{\core}{\ensuremath{\mathcal{Q}\textsc{wire}}\xspace}
\newcommand{\hostname}{\textsc{host}}
\newcommand{\host}{\ensuremath{\hostname}\xspace}
\newcommand{\qhost}{\ensuremath{\mathcal{Q}\hostname}\xspace}

\newcommand{\CONS}{\ensuremath{\!::\!}}

%% COMMENTS 
\newtoggle{comments}
\togglefalse{comments}

\iftoggle{comments}{
  \newcommand{\dmitri}[1]{\textbf{\textcolor{red}{[ #1 --- Dmitri]}}}
  \newcommand{\steve}[1]{\textbf{\textcolor{olive}{[ #1 --- Steve]}}}
  \newcommand{\william}[1]{\textbf{\textcolor{blue}{[ #1 --- William]}}}
    \newcommand{\christine}[1]{\textbf{\textcolor{purple}{[ #1 --- Christine]}}}

  \newcommand{\fixme}[1]{\textbf{\textcolor{red}{[ Fixme: #1]}}}
  \newcommand{\note}[1]{\textbf{\textcolor{green}{[ Note: #1 ]}}}
  \newcommand{\todo}[1]{\textbf{\textcolor{purple}{[ TODO: #1 ]}}}
}{
  \newcommand{\dmitri}[1]{}
  \newcommand{\steve}[1]{}
  \newcommand{\william}[1]{}

  \newcommand{\fixme}[1]{}
  \newcommand{\note}[1]{}
  \newcommand{\todo}[1]{}
}
%% END COMMENTS

